Alpha Backgrounds for HPGe Detectors in Neutrinoless Double-Beta Decay Experiments

The Majorana Experiment will use arrays of enriched HPGe detectors to search for the neutrinoless double-beta decay of 76Ge. Such a decay, if found, would show lepton-number violation and confirm the Majorana nature of the neutrino. Searches for such rare events are hindered by obscuring backgrounds which must be understood and mitigated as much as possible. A potentially important background contribution to this and other double-beta decay experiments could come from decays of alpha-emitting isotopes in the 232Th and 238U decay chains on or near the surfaces of the detectors. An alpha particle emitted external to an HPGe crystal can lose energy before entering the active region of the detector, either in some external-bulk material or within the dead region of the crystal. The measured energy of the event will only correspond to a partial amount of the total kinetic energy of the alpha and might obscure the signal from neutrinoless double-beta decay. A test stand was built and measurements were performed to quantitatively assess this background. We present results from these measurements and compare them to simulations using Geant4. These results are then used to measure the alpha backgrounds in an underground detector in situ. We also make estimates of surface contamination tolerances for double-beta decay experiments using solid-state detectors.

==> Bulk.tex <==
\subsection{Bulk-Alpha Backgrounds}
\label{sec:Bulk}



\subsection{Analytic Model}

A model, similar to that of the surface-type detector response, was constructed
to describe bulk-type data on the detector.  The typical range of an alpha in
solid materials of interest (copper, lead, gold, germanium) is on the order 10's
of $\mu$m.  Thus only the outer portion of material facing the crystal will
contribute alpha backgrounds.  An alpha of original energy $E_0$, emitted in an
external-bulk material at a depth $d$ from the material surface at an angle
$\theta$ with respect to the normal of that surface, will then lose an average
energy similar to Eq. \ref{eq:DeltaE} where $dE/dx$ is a function of the alpha's
energy and distance traveled.  Similarly, energy straggling will widen the
resulting peak. The spectrum from an alpha of initial energy $E_{0}$ at a depth
$d$ emitted at an angle $\theta$ would then be given as

\begin{align}
\label{eq:ThModel}
f\left(E,E_{0},d,\theta\right) &= \frac{1}{\sqrt{2\pi}\sigma} \exp\left(-\frac{E +
E_{0} -\Delta E}{2\sigma^2} \right) \\ \notag
\sigma^2 &=  4\pi N_{a}r^2_{e}(m_{e}c^2)^2\rho\frac{Z}{A}\Delta x \\ \notag
&= 289.9 \Delta x \\ \notag
\Delta E &= \int^{d/\cos\theta}_0 \frac{dE}{dx}dx  .
\end{align}

\noindent where we once again assume a Bohr model of energy straggling and
$\sigma^2$ is calculated using $\rho$, $Z$, and $A$ of thorium. Deviations from
the Bohr model are discussed in Section \ref{sec:Impact}.  While $f$
could be described with an exponentially-modified gaussian as in Section
\ref{sec:Surface}, such details are washed out in practice because of the
continuum nature of the energy spectrum as
$f$ is integrated over $\theta$ and $d$.

The model spectrum for a particular decay is then found by integrating Eq.
\ref{eq:ThModel} over $\theta$ and $d$.  Values for $dE/dx$ were taken from
alpha stopping-power and range tables \cite{Astar}, and this integration was
performed for all the alphas in the \iso{232}{Th} decay chain (Table
\ref{tab:Th232Source}). The corresponding energy spectra were then summed,
assuming the chain is in secular equilibrium.  This assumption is valid in our
comparison with our data because all alpha decays in the \iso{232}{Th} chain,
except the first, happen within days of each other (Table
\ref{tab:Th232Source}).  The first alpha decay (\iso{232}{Th}) emits a 4 MeV
alpha which is not discernable below the beta continuum in the data set. 

This model was compared with the data set (Fig. \ref{fig:ThoriumSpectrum}).  The
fast alpha decay (300 ns) of \iso{212}{Po}, coming after the beta decay of
\iso{212}{Bi}, occasionally results in pileup in the detector of the alpha (8.8
MeV) and the beta (endpoint 2252 keV, intensity 55.4\%).  To treat this, the
\iso{212}{Po} alpha spectrum was convolved with the beta spectrum of
\iso{212}{Bi}.  A fit was performed to the data consisting of a histogram with
all of the alpha spectra except \iso{212}{Po}, a histogram with an unmodified
\iso{212}{Po} spectrum, a histogram with a convolved \iso{212}{Po} spectrum, and
a cosmic ray background parametrized as $f_{CR} = \alpha(1+\beta e^{-\gamma
E})$, with the parameters $\alpha$, $\beta$, $\gamma$, and the proportions of the
different histograms determined in the fit.  The resultant model spectrum is
compared with the data in Fig. \ref{fig:ThoriumSpectrum}.

The thorium wire geometry was simulated in MaGe, and the output was subjected to
the same correction convolution as the collimation data.  The simulated spectrum
is compared with the data and model in Fig. \ref{fig:ThoriumSpectrum}.

\begin{figure}[h]
\includegraphics[width=0.49\textwidth]{BulkCompare}
%\includegraphics[width=0.49\textwidth]{LabeledThorium}
\caption{High-energy spectrum of thorium wire on HPGe surface.  Characteristic
steps corresponding to initial kinetic energies of alphas in \iso{232}{Th} decay
chains are marked.  The lower-energy spectrum is dominated by gammas from the
chain, and the lines visible above 3 MeV are double and triple coincidences of
the 583 keV, 2615 keV, and 511 
keV gammas from \iso{208}{Tl}.{\color{red} yep, i realize it has no label.
trying to figure out why the model is'nt replicating the step endpoints well
(the model steps are higher in energy and steeper than the data)}.}
\label{fig:ThoriumSpectrum}
\end{figure}

{\color{red} Validation of the bulk sectin is turning out to be more complicated
than I'd anticipated.  Need to decide what's useful to extract from this.}

